AdapTable: Test-Time Adaptation for Tabular Data via Shift-Aware Uncertainty Calibrator and Label Distribution Handler

In real-world scenarios, tabular data often suffer from distribution shifts that threaten the performance of machine learning models. Despite its prevalence and importance, handling distribution shifts in the tabular domain remains underexplored due to the inherent challenges within the tabular data itself. In this sense, test-time adaptation (TTA) offers a promising solution by adapting models to target data without accessing source data, crucial for privacy-sensitive tabular domains. However, existing TTA methods either 1) overlook the nature of tabular distribution shifts, often involving label distribution shifts, or 2) impose architectural constraints on the model, leading to a lack of applicability. To this end, we propose AdapTable, a novel TTA framework for tabular data. AdapTable operates in two stages: 1) calibrating model predictions using a shift-aware uncertainty calibrator, and 2) adjusting these predictions to match the target label distribution with a label distribution handler. We validate the effectiveness of AdapTable through theoretical analysis and extensive experiments on various distribution shift scenarios. Our results demonstrate AdapTable's ability to handle various real-world distribution shifts, achieving up to a 16% improvement on the HELOC dataset.

==> sections/9_checklist.tex <==
\section{Reproducibility Checklist}
\begin{itemize}
    \item \textbf{Includes a conceptual outline and/or pseudocode description of AI methods introduced} (yes)
    
    \item \textbf{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results} (yes)
    
    \item \textbf{Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper} (yes)
    
    \item \textbf{Does this paper make theoretical contributions?} (yes)
    \begin{itemize}
        \item If yes, please complete the list below.
        \begin{itemize}
            \item All assumptions and restrictions are stated clearly and formally. (yes)
            
            \item All novel claims are stated formally (e.g., in theorem statements). (yes)
            
            \item Proofs of all novel claims are included. (yes)
            
            \item Proof sketches or intuitions are given for complex and/or novel results. (yes)
            
            \item Appropriate citations to theoretical tools used are given. (yes)
            
            \item All theoretical claims are demonstrated empirically to hold. (yes)
            
            \item All experimental code used to eliminate or disprove claims is included. (NA)
        \end{itemize}
    \end{itemize}
    
    \item \textbf{Does this paper rely on one or more datasets?} (yes)
    \begin{itemize}
        \item If yes, please complete the list below.
        \begin{itemize}
            \item A motivation is given for why the experiments are conducted on the selected datasets. (yes)
            
            \item All novel datasets introduced in this paper are included in a data appendix. (NA)
            
            \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)
            
            \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
            
            \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
            
            \item All datasets that are not publicly available are described in detail, with an explanation of why publicly available alternatives are not scientifically satisfying. (NA)
        \end{itemize}
    \end{itemize}
    
    \item \textbf{Does this paper include computational experiments?} (yes)
    \begin{itemize}
        \item If yes, please complete the list below.
        \begin{itemize}
            \item Any code required for pre-processing data is included in the appendix. (yes)
            
            \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)
            
            \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
            
            \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. (yes)
            
            \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
            
            \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
            
            \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
            
            \item This paper states the number of algorithm runs used to compute each reported result. (yes)
            
            \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
            
            \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (partial)
            
            \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
            
            \item This paper states the number and range of values tried per (hyper-)parameter during the development of the paper, along with the criterion used for selecting the final parameter setting. (yes)
        \end{itemize}
    \end{itemize}
\end{itemize}

==> tables/ablation_study.tex <==
\begin{table}[!ht]
\centering
\caption{
Ablation study of AdapTable decomposed into the components, where \emph{SUC} indicates shift-aware uncertainty calibrator.
}
\label{table:ablation}
\begin{adjustbox}{width=.8\linewidth}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{lcccc}
    \toprule
    
    Method & $\text{CMC}_{\text{Numerical}}$ & $\text{CMC}_{\text{Categorical}}$ & MFEAT-PIXEL & HELOC \\ \hline

    Source & 59.7 {$\pm$ 1.6} & 58.1 {$\pm$ 0.8} & 96.0 {$\pm$ 0.1} & 47.0 {$\pm$ 1.6} \\ % \cdashline{1-5}
    
    w/o SUC & 61.9 {$\pm$ 0.7} & 61.4 {$\pm$ 1.2} & 97.2 {$\pm$ 0.1} & 61.7 {$\pm$ 2.2} \\
    
    MLP SUC & 64.0 {$\pm$ 0.9} & 62.6 {$\pm$ 1.3} & 97.4 {$\pm$ 0.1} & 62.5 {$\pm$ 0.6} \\ % \hline
    
    AdapTable & \textbf{65.6 {$\pm$ 1.6}} & \textbf{64.2 {$\pm$ 2.4}} & \textbf{97.8 {$\pm$ 0.2}} & \textbf{64.5 {$\pm$ 0.3}} \\ 
    
    \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/main_common_corruption.tex <==
\begin{table*}[!t]
\caption{
    The average accuracy (\%) and their corresponding standard errors of both supervised models and TTA baselines with MLP backbone architecture across three datasets from OpenML-CC18 benchmark~\citep{openml_benchmark}, each corrupted with 6 different common corruptions: Gaussian noise, uniform noise, random column drop, random missing, numerical column shifts, categorical column shifts. The results are reported over three different random seeds.
}
\label{table:second_table}
\centering
\setlength{\columnsep}{1pt}
\begin{adjustbox}{width=0.9\linewidth}
\begin{tabular}{@{\extracolsep{1pt}}clccccccccc@{}}
\toprule

& \multirow{2}{*}{Method} & \multicolumn{3}{c}{{CMC}} & \multicolumn{3}{c}{{MFEAT-PIXEL}} & \multicolumn{3}{c}{{DNA}} \\

\cline{3-5}\cline{6-8}\cline{9-11}\rule{0pt}{2.2ex}
& & Acc. & bAcc. & F1 & Acc. & bAcc. & F1  & Acc. & bAcc. & F1 \\
\cline{2-11}
\rule{0pt}{2.5ex}
\multirow{6}{*}{\rotatebox{90}{Supervised}}
    & k-NN     & 47.9 {$\pm 1.7$} & 45.4 {$\pm 1.3$} & 44.0 {$\pm 1.3$} & 96.2 {$\pm 0.5$}       & 96.1 {$\pm 0.5$}        & 95.8 {$\pm 0.6$}      & 79.3 {$\pm 1.6$} & 77.0 {$\pm 1.1$} & 77.8 {$\pm 1.2$} \\
            
    & LR        & 49.0 {$\pm 1.4$} & 46.3 {$\pm 1.3$} & 42.8 {$\pm 1.3$} & \bf 96.8 {$\pm 0.5$}       & \bf 96.6 {$\pm 0.5$}        & \bf 96.6 {$\pm 0.5$}      & 89.4 {$\pm 2.0$} & 87.9 {$\pm 1.7$} & 87.8 {$\pm 2.1$} \\
    
    & RF        & 51.4 {$\pm 1.5$} & 48.5 {$\pm 1.3$} & 44.5 {$\pm 1.4$} & 96.5 {$\pm 0.3$}       & 96.3 {$\pm 0.4$}        & 96.3 {$\pm 0.4$}      & 91.1 {$\pm 2.0$} & 90.7 {$\pm 1.6$} & 89.2 {$\pm 2.1$} \\
    
    & XGBoost & \bf 52.9 {$\pm 2.0$} & \bf 49.7 {$\pm 1.7$} & 47.1 {$\pm 1.7$} & 94.2 {$\pm 0.6$}       & 94.0 {$\pm 0.8$}        & 93.9 {$\pm 0.8$}      & 91.7 {$\pm 2.1$} & 91.1 {$\pm 1.8$} & 90.2 {$\pm 3.2$} \\
    
    & CatBoost & 51.9 {$\pm 2.0$} & 49.0 {$\pm 1.8$} & 47.4 {$\pm 1.8$} & 96.5 {$\pm 0.4$}       & 96.3 {$\pm 0.5$}        & 96.3 {$\pm 0.5$}      & 91.8 {$\pm 2.0$} & 90.7 {$\pm 1.8$} & 90.4 {$\pm 2.1$} \\
    
    & + {AdapTable} & 52.4 {$\pm 1.6$} & 49.3 {$\pm 0.6$} & \bf 48.6 {$\pm 0.7$} & 96.7 {$\pm 0.5$}       & \bf 96.6 {$\pm 0.5$}        & 96.5 {$\pm 0.5$}      & \bf 94.6 {$\pm 1.1$} & \bf 92.9 {$\pm 1.8$} & \bf 93.8 {$\pm 1.5$} \\

    \cline{2-11}
    \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
\multirow{8}{*}{\rotatebox{90}{MLP}}
    & Source & 53.5 {$\pm 1.6$} & 47.9 {$\pm 1.4$} & 47.9 {$\pm 1.5$} & 96.4 {$\pm 0.3$}       & 96.4 {$\pm 0.4$}        & 96.3 {$\pm 0.4$}      & 91.4 {$\pm 1.5$} & \bf 90.1 {$\pm 1.5$} & 90.0 {$\pm 1.5$} \\
    
    & PL        & 54.1 {$\pm 2.0$} & 47.8 {$\pm 1.5$} & 47.8 {$\pm 1.5$} & 96.4 {$\pm 0.3$}       & 96.5 {$\pm 0.3$}        & 96.3 {$\pm 0.4$}      & 90.9 {$\pm 1.5$} & 89.5 {$\pm 1.8$} & 89.4 {$\pm 1.5$} \\
    
    & TTT++     & 52.7 {$\pm 1.7$} & 47.2 {$\pm 1.4$} & 47.2 {$\pm 1.8$} & 95.8 {$\pm 0.4$}       & 95.6 {$\pm 0.5$}        & 95.5 {$\pm 0.5$}      & 89.5 {$\pm 1.3$} & 86.6 {$\pm 1.5$} & 87.6 {$\pm 1.5$} \\
    
    & TENT     & 54.1 {$\pm 2.0$} & 47.5 {$\pm 1.4$} & 47.5 {$\pm 1.5$} & 96.5 {$\pm 0.4$}       & 96.5 {$\pm 0.3$}        & 96.4 {$\pm 0.3$}      & 90.3 {$\pm 1.4$} & 88.7 {$\pm 1.9$} & 88.6 {$\pm 1.7$} \\
    
    & EATA      & 53.8 {$\pm 1.7$} & 48.1 {$\pm 1.4$} & 48.1 {$\pm 1.5$} & 96.4 {$\pm 0.4$}       & 96.5 {$\pm 0.4$}        & 96.3 {$\pm 0.4$}      & 91.4 {$\pm 1.4$} & \bf 90.1 {$\pm 1.7$} & 90.0 {$\pm 1.5$} \\
    
    & SAR      & 48.0 {$\pm 2.0$} & 37.7 {$\pm 0.7$} & 37.7 {$\pm 0.7$} & 65.6 {$\pm 5.0$}       & 63.8 {$\pm 5.1$}        & 62.8 {$\pm 5.8$}      & 62.6 {$\pm 3.1$} & 59.8 {$\pm 2.8$} & 55.2 {$\pm 3.5$} \\
    
    & LAME      & 49.6 {$\pm 4.4$} & 40.3 {$\pm 3.2$} & 40.3 {$\pm 3.1$} & 95.9 {$\pm 0.7$}       & 95.8 {$\pm 0.7$}        & 95.7 {$\pm 0.7$}      & 74.9 {$\pm 5.1$} & 63.6 {$\pm 5.8$} & 63.8 {$\pm 9.1$} \\
    
    & {AdapTable} & \bf 55.7 {$\pm 2.4$} & \bf 50.3 {$\pm 1.8$} & \bf 50.2 {$\pm 1.7$} & \bf 97.8 {$\pm 0.4$}       & \bf 97.5 {$\pm 0.4$}        & \bf 97.4 {$\pm 0.4$}      & \bf 95.0 {$\pm 0.6$} & 89.9 {$\pm 1.8$} & \bf 92.1 {$\pm 0.9$} \\

    \bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}
